CSPO: Cross-Market Synergistic Stock Price Movement Forecasting with Pseudo-volatility Optimization

The stock market, as a cornerstone of the financial markets, places forecasting stock price movements at the forefront of challenges in quantitative finance. Emerging learning-based approaches have made significant progress in capturing the intricate and ever-evolving data patterns of modern markets. With the rapid expansion of the stock market, it presents two characteristics, i.e., stock exogeneity and volatility heterogeneity, that heighten the complexity of price forecasting. Specifically, while stock exogeneity reflects the influence of external market factors on price movements, volatility heterogeneity showcases the varying difficulty in movement forecasting against price fluctuations. In this work, we introduce the framework of Cross-market Synergy with Pseudo-volatility Optimization (CSPO). Specifically, CSPO implements an effective deep neural architecture to leverage external futures knowledge. This enriches stock embeddings with cross-market insights and thus enhances the CSPO's predictive capability. Furthermore, CSPO incorporates pseudo-volatility to model stock-specific forecasting confidence, enabling a dynamic adaptation of its optimization process to improve accuracy and robustness. Our extensive experiments, encompassing industrial evaluation and public benchmarking, highlight CSPO's superior performance over existing methods and effectiveness of all proposed modules contained therein.

==> method/method_backup.tex <==
% \section{\model~ Methodology}

% \subsection{Overview}
% TBC


% \subsection{\textbf{Time Series Information Encoding}}
% In this work, we use DeepFFM~\cite{xx} to process the raw stock price-volume features and map them into a high-dimensional space. After modeling the feature interactions, the output is compressed back to a $d$-dimensional feature vector.

% \begin{equation}
% \tilde{S}, \tilde{C}, \tilde{E} \in \mathbb{R}^{t \times d}
% \end{equation}%


% The FFN feature extraction can be expressed as:
% \begin{equation}
% \tilde{S}_{1:t} = \text{FFN}(S_{1:t})
% \end{equation}%
% \begin{equation}
% \tilde{C}_{1:t} = \text{FFN}(C_{1:t})
% \end{equation}%
% \begin{equation}
% \tilde{E}_{1:t} = \text{FFN}(E_{1:t})
% \end{equation}%

% Since time series data from different market have distinct semantics, we first use market-specific transformer blocks to extract the awareness of the dynamic market monetary liquidity and asset pricing.
% \begin{equation}
% S^* = \textit{meanPooling}\left( \mathbf{\textit{TransformerEncoder}_S}(\tilde{S}_{1:t}) \right)
% \end{equation}%
% \begin{equation}
% C^* = \textit{meanPooling}\left( \mathbf{\textit{TransformerEncoder}_C}(\tilde{C}_{1:t}) \right)
% \end{equation}%
% \begin{equation}
% E^* = \textit{meanPooling}\left( \mathbf{\textit{TransformerEncoder}_E}(\tilde{E}_{1:t}) \right)
% \end{equation}%


% \subsection{Stock Volatility Estimation}
% {\todo Volatility or Uncertainty?}

% \subsection{{\normalfont\texttt{Funnel-Transformer}} for Price Forecasting}

% \subsubsection{\textbf{Decoder Only Bi-Graph Transformer}}
% Here, we design a new Graph-Transformer structure to model the dynamic one-way interconnections between stocks and a decoder-only alike structure, serving as a Bipartite Graph-Transformer (BiGT), to model the relationships between upstream and downstream assets and macroeconomic liquidity with stocks. 


% The scaled dot-product attention is computed as:

% \begin{equation}
% \text{BiAtt}(I,M) = \frac{1}{\sqrt{d}} \textit{Softmax}\left( W_QI \cdot W_KM \right) \cdot W_VM
% \end{equation}%

% The Transformer applies multiple attention heads in parallel:
% \begin{equation}
% \text{BiMHA}(I,M) = \text{Concat}(\text{BiAtt}_1, \text{BiAtt}_2, \dots, \text{BiAtt}_h)W^O
% \end{equation}%


% The Transformer architecture we propose consists of $N$ identical encoder layers, each represented as follows:
% \begin{equation}
% \text{I}_{i+1} = \text{LayerNorm}(\text{I}_i + \text{FFN}(\text{BiMHA}(\text{I}_i, M)))
% \end{equation}%


% The final output of the full model is obtained after 
% \begin{equation}
% I^* = \text{I}_N = \text{LayerNorm}(\text{I}_{N-1} + \text{FFN}(\text{BiMHA}(\text{I}_{N-1}, M)))
% \end{equation}%

% Finaly, 

% \begin{equation}
% I^* = \textit{BiGT}\left(I, M\right)
% \end{equation}%






% \subsubsection{\textbf{Hierarchical Graph Transformer}}

% \textbf{Graph Position Encoding} 
% \begin{equation}
% PE_{c} = \textit{BiGT}\left( S^*, C^* \right)
% \end{equation}%
% \begin{equation}
% PE_{e} = \textit{BiGT}\left( S^*, E^* \right)
% \end{equation}%
% \begin{equation}
% PE^* = PE_{c} + PE_{e}
% \end{equation}%

% \textbf{Graph Transformer} 
% \begin{equation}
% S^* = \textit{GraphTransformer}\left( S^* + PE^* \right)
% \end{equation}%


% The final output combines the stock relationship, asset pricing, and liquidity awareness components to generate a comprehensive market view. This fusion of multiple dimensions of financial data enhances predictive power, providing a robust framework for asset allocation and risk management in complex financial systems.



% \subsection{\textbf{Volatility-aware Model Optimization}}
% \subsubsection{\textbf{Uncertainty Modeling}}
% \begin{equation}
% Var = \textit{meanPooling}\left( \mathbf{\textit{TransformerEncoder}_V}(\tilde{S}_{1:t}) \right)
% \end{equation}%

% Finally, formed the entire model as Triple-C Market Transformer (\textit{TCMT})
% \subsubsection{\textbf{Bayesian NN}}

% Here we actually modeling transformed std refer to paper Bayesian for CV
% \begin{equation}
% Mu_a, Var_a = \textit{TCMT}_a\left( S_{1:t}, C_{1:t}, E_{1:t} \right)
% \end{equation}%
% \begin{equation}
% Mu_b, Var_b = \textit{TCMT}_b\left( S_{1:t}, C_{1:t}, E_{1:t} \right)
% \end{equation}%
% \begin{equation}
% Prediction = \textit{meanPooling}\left( Mu_a + Mu_b \right)
% \end{equation}%

% \subsection{\textbf{Loss Term}}

% MSE
% Bayesian Loss
